Abstraction-based Probabilistic Stability Analysis of Polyhedral Probabilistic Hybrid Systems

In this paper, we consider the problem of probabilistic stability analysis of a subclass of Stochastic Hybrid Systems, namely, Polyhedral Probabilistic Hybrid Systems (PPHS), where the flow dynamics is given by a polyhedral inclusion, the discrete switching between modes happens probabilistically at the boundaries of their invariant regions and the continuous state is not reset during switching. We present an abstraction-based analysis framework that consists of constructing a finite Markov Decision Processes (MDP) such that verification of certain property on the finite MDP ensures the satisfaction of probabilistic stability on the PPHS. Further, we present a polynomial-time algorithm for verifying the corresponding property on the MDP. Our experimental analysis demonstrates the feasibility of the approach in successfully verifying probabilistic stability on PPHS of various dimensions and sizes.

==> char.tex <==
\section{Alternate Characterization of Almost Sure Convergence}
We now provide an alternate characterization for almost sure convergence of $\rmdp$. 
With this characterization, we will be able to use existing results (from~\cite{das2022stability}) that will eventually help us to solve the original problem.
First, let us associate a notion of payoff to each infinite path. 
In general, payoff is a mapping from the set of infinite paths to $\real$. We define mean payoff of an infinite path as the limit supremum of the average weight of the path.
\begin{comment}
We say a payoff $\phi$ is prefix independent if for any $u\in\fpath{\Mw}$ and any $v\in\ipath{\Mw}$, $\phi(uv) = \phi(v)$. 
Also, a payoff $\phi$ is submixing if for any infinite sequence of finite paths $u_0,v_0,u_1,v_1,\dots$, $\phi(u_0v_0u_1v_1\dots)\leq\max\{\phi(u_0u_1\dots),\phi(v_0v_1\dots)\}$. 
We now define the mean payoff function which is both prefix independent and submixing~\cite{gimbert2007pure}.
\end{comment}
\begin{definition}
[Mean Payoff] For a $\rmdp$ $\Mw$, the mean payoff $\meanpay$ is a function from $\ipath{\Mw}$ to $\real$ defined as,
\[\meanpay(\Path) = \limsup_{n\rightarrow\infty}\frac{\weight(\Path[0:n])}{n}.\]
\end{definition}
We characterize convergence of $\rmdp$ using mean payoff.
We know (from~\cite{das2022stability}) that weight of an infinite path is $-\infty$ if and only if its mean payoff is strictly negative. Hence, we have the following theorem:
\begin{theorem}[Characterization of Almost Sure Convergence]\label{thm:mean_conv_cond}
 A $\rmdp$ $\Mw$ is almost surely convergent iff for any policy $\policy\in\polset$, mean payoff of an infinite path is strictly negative with probability $1$, i.e., for all $\policy\in\polset$,
\[
\prob_\policy\{\Path\in\ipath{\Mw}:\meanpay(\Path)<0\}= 1.
\]
\end{theorem}
Thus to check if a $\rmdp$ is almost surely convergent, it is enough to check whether mean payoff of an infinite path is almost surely negative under any policy. We will show that, this condition is true when mean payoff is almost surely negative under all memoryless policies. Since $\rmdp$ associated with a memoryless policy is a $\rdtmc$, let us discuss a method for deciding almost sure convergence of a $\rdtmc$ first.


==> decide.tex <==
\section{Decidability of Almost Sure Convergence}

Since there are only finitely many memoryless policies for a $\rmdp$, we have an algorithm for deciding almost sure convergence of $\rmdp$.
Basically, for a $\rmdp$ $\Mw$, we can check if the underlying $\rdtmc$ $(\Mw,\policy)$ is almost surely convergent for every memoryless policy $\policy$.
We describe this procedure in Algorithm~\ref{algo:eps-conv}.

\begin{algorithm}[ht]
\begin{algorithmic}[1]
    \renewcommand{\algorithmicrequire}{\textbf{Input:}}
    \renewcommand{\algorithmicensure}{\textbf{Output:}}
	\Require{A $\rmdp$ $\Mw = (\states,\acts,\trans,\weight)$}
	\Ensure Yes/No
	
	\For{each memoryless policy $\policy$}
	    \For{each $\bscc$ $\B$ of the $\rdtmc$ $(\Mw,\policy)$}
            \State $w\gets$ effective weight of $\rdtmc$ induced by $\B$~\cite{das2022stability}
            \If{$w\geq 0$}
                \State Return No
	       \EndIf
        \EndFor
    \EndFor
    \State Return Yes
\end{algorithmic}
\caption{Deciding Almost Sure Convergence of WMDP}\label{algo:eps-conv}
\end{algorithm}


\begin{theorem}\label{algo:correctness}
[Correctness of Algorithm~\ref{algo:eps-conv}] Algorithm~\ref{algo:eps-conv} returns ``Yes" iff the input $\rmdp$ $\Mw$ is almost surely convergent.
\end{theorem}

\begin{proof}
From Theorem~\ref{thm:suff-conv} we know that, $\Mw$ is almost surely convergent iff probability of the set of infinite paths having negative mean payoff is $1$ for all memoryless policies. 
Now, $\Mw$ associated with a memoryless policy $\policy$ generates a $\rdtmc$.
By definition, the $\rdtmc$ $(\Mw,\policy)$ is almost surely convergent iff almost surely all infinite paths of $\Mw$ have negative mean payoff under $\policy$. 
By Theorem~\ref{thm:as-conv-dtmc}, this happens iff effective weight of each $\rdtmc$ induced by a $\bscc$ of $(\Mw,\policy)$ is less than $0$. 
This is exactly the condition when Algorithm~\ref{algo:eps-conv} returns ``Yes", i.e., Algorithm~\ref{algo:eps-conv} returns ``Yes" iff $\Mw$ is almost surely convergent.\qed
\end{proof}

==> drw.tex <==
\section{Detailed Related Work}
\subsection{Markov Decision Process}

\begin{enumerate}
\item {\bf Title:} Games and MDP with Mean Payoff Parity and Energy Parity Objectives (MEMICS 2011)\\
{\bf Author:} Krishnendu Chatterjee et. al.\\
{\bf Summary:}\\
An MDP is a set of states with some of the states designated to player 1 and the others to nature. After player 1 makes a move, the nature takes control and the next state is chosen probabilistically based on the previous state and action taken by player 1. A reward is associated to each state transition $(s,a,t)$, where $s$ is the current state, $a$ the action chosen by player 1 and $t$ the next state obtained from the probability distribution.

An infinite path is an infinite sequence of consecutive transitions. Mean payoff of an infinite path $\Path$ is given by $MP(\Path) = \liminf_{n\rightarrow\infty}n^{-1}\sum_{i=1}^n r(q_i,q_{i+1})$, where $(q_i,q_{i+1})$ is the $i^{th}$ transition of $\Path$.

\textbf{Mean payoff objective:} Given a threshold $\nu$, the mean payoff objective is the set $\{\Path\mid MP(\Path)\geq\nu\}$. Player 1 is said to have an almost sure winning strategy $\policy$, if probability of mean payoff objective is $1$, i.e., $\prob_\policy\{\Path\mid MP(\Path)\geq \nu\}=1$. 

\textbf{Problem:} Given an MDP and an objective, the goal is to decide whether an almost sure winning strategy exists for player 1. The decision problem for existence of almost sure winning strategy for mean payoff objective can be solved through linear programming, that is, in polynomial time.
\vspace{10pt}
\item \textbf{Title:} Markov Decision Process (book 1994)\\
\textbf{Author:} Martin L. Puterman\\
\textbf{Summary:}\\
An MDP consists of a set of states and a set of actions. At each step an action is chosen non-deterministically and the next state is guessed according to a fixed probability based on the current state and the chosen action. 

A transition is a triple $(s,a,t)$ where $s$ is the current state, $a$ is the chosen action and $t$ is the next state chosen probabilistically according to $s,a$. An immediate reward is associated to every transition. 
A average reward is associated to an infinite path as the average reward of individual transitions as number of steps goes to $\infty$.

A strategy associates a probability of choosing the next action given a finite history.
By solving an MDP with average reward criterion, we mean to find a strategy that maximizes the expected average reward under all strategies.
A unichain MDP is one which under any memoryless strategy, provides one recurrent class and a possibly empty transient set of states.
It is shown that unichain MDPs can be solved by a memoryless strategy that can be found by solving a linear program.

\vspace{10pt}

\item \textbf{Title:} Efficient Strategy Iteration for Mean Payoff in MDP (ATVA 2017)\\
\textbf{Author:} Jan Kretinsky et. al.\\
\textbf{Summary:}\\
MDP is defined as before. At each state, taking an action provides an immediate reward which does not depend on the next state. A strategy is deterministic in the sense that the next action is chosen deterministically provided the history. The gain of an infinite path is defined as the liminf of the expected average reward.

\textbf{Problem:} Find the maximum possible gain under any strategy and the strategy that achieves this gain.\\
\textbf{Algorithm:} The problem is solved using strategy iteration.
\begin{itemize}
\item Choose a strategy arbitrarily
\item Evaluate the strategy, i.e., find its gain ($g$) and bias ($b$)
\begin{align*}
&g(s) = \sum_{s'\in S}\Delta(s,s')g(s')=E_\Delta(g,s) \quad\forall s\in S\\
&b(s) = \sum_{s'\in S}\Delta(s,s')b(s') + r(s) - g(s) = E_\Delta(b,s) + r(s) - g(s) \quad \forall s\in S.
\end{align*}
Here $S$ is the set of states, $\Delta(s,s')$ is the probability of choosing $s'$ once $s$ and action is known. Here action is omitted as it is clear from the chosen strategy. $r(s)$ is the immediate reward gained from state $s$, here also the action is omitted.

\item Improve each action choice greedily until no more improvement is possible.
\end{itemize}
Multiple ways of efficiently evaluating gain and bias have been discussed in the paper. Algorithms are tested on virus environment that encodes virus spreading through a network.

\vspace{10pt}

\item \textbf{Title:} Reinforcement Learning Algorithms for Average-Payoff MDPs (AAAI 1994)\\
\textbf{Author:} Satinder P. Singh\\
\textbf{Summary:}\\
MDP, strategy and immediate reward are defined as before. Average payoff of an infinite path is also defined as before. \\
\textbf{Problem:} Given an MDP, find the policy that maximizes the expected average payoff.

The paper discusses several value iteration and policy iteration algorithms to find the optimal policy.

\textbf{Value iteration example:}\\
\begin{align*}
&V_{t+1}(x_t) = (1-\alpha_t(x_t))V_t(x_t) + \alpha_t(x_t)(R(x_t,\pi(x_t))+V_t(x_{t+1})-\rho_t)\\
&\text{where }\rho_0=0\text{ and}\\
&\rho_{t+1} = (1-\beta(t))\rho_t + \beta(t)[\mathcal{B}_\pi(V_t)(x_t)-V_t(x_t)]
\end{align*}
Here $\alpha,\beta$ are learning rates, $R$ is the immediate reward function, $\mathcal{B}_\pi$ is the DP operator associated to strategy $\pi$. $V$ gives the next value of the state $x$, that is, maximum expected average payoff when an infinite path starts from $x$.

\textbf{Policy iteration example:}\\
\begin{align*}
&Q_{t+1}(x_t,a_t) = (1-\alpha_t(x_t,a_t))Q_t(x_t,a_t) + \alpha_t(x_t,a_t)(\mathcal{B}(Q_t)(x_t,a_t) - \rho_t)\\
&\rho_{t+1} = (1-\beta_t)\rho_t + \beta_t(\mathcal{B}(Q_t)(x_t,a_t) - Q_t(x_t,a_t))
\end{align*}
This is a typical $Q$-learning algorithm where the next $Q$-value is calculated based on previous $Q$-value and the current chosen strategy. $\alpha$, $\beta$, $\mathcal{B}$ are defined as before.

The paper compares the value iteration and policy iteration algorithms on several randomly constructed MDPs and publish the results graphically.

\vspace{10pt}

\item \textbf{Title:} Strategy Complexity of Mean Payoff, Total Payoff and Point Payoff Objectives in Countable MDPs (2021)\\
\textbf{Author:} Richard Mayr et. al.\\
\textbf{Summary:}
MDP, strategy and immediate rewards are defined as before. Here MDP has countably infinite states.\\
\textbf{Total payoff:} For an infinite path $\Path$, total payoff is the $\liminf$ of the sequence $\{\sum_{i=1}^n r_i\}_{n\in\nat}$ where $r_i$ is the immediate reward observed at $i^{th}$ transition of the path.\\
\textbf{Mean payoff:} For an infinite path $\Path$, mean payoff is the $\liminf$ of the sequence $\{n^{-1}\sum_{i=1}^n r_i\}_{n\in\nat}$ where $r_i$ is the immediate reward observed at $i^{th}$ transition of the path.\\
\textbf{Problem:} 
Find a strategy that maximizes the probability that the payoff is at least $0$, i.e., $\sup_{\pi\in\Pi}\prob_\pi\{\Path\mid\text{mean payoff of }\Path\geq 0\}$.

The paper discusses memory requirement for solving this problem. Some problems are solvable by memoryless strategies, whereas other problems require infinite memory in form of step counter and reward counter.

\vspace{10pt}

\item \textbf{Title:} Pure Stationary Optimal Strategies for MDPs (HAL 2007)\\
\textbf{{Author:}} Hugo Gimbert\\
\textbf{Summary:}\\
MDP, immediate reward and strategy are defined as before. Payoff associated to an infinite path is a mapping from the infinite path to real. The mean payoff is the average of all immediate rewards gathered while traversing the path. A payoff is prefix-independent if its value does not depend on any finite prefix. It is submixing if we can write an infinite path $\Path$ as a concatenation of finite paths $\Path=u_0v_0u_1v_1\dots$ in any way but payoff associated to $\Path$ is upper bounded by maximum of payoff associated to $u_0u_1\dots$ and payoff associated to $v_0v_1\dots$. The paper shows that for prefix-independent and submixing payoffs, there is a memoryless deterministic strategy that maximizes expected payoff.

\vspace{10pt}

\item \textbf{Title:} MDP and Stochastic Games with total effective payoff (AOR 2018)\\
\textbf{Author:} Endre Boros et. al.\\
\textbf{Summary:}\\
MDP, strategy and immediate reward are defined as before. Two types of payoff are associated to infinite paths:\\
\textbf{Mean payoff:} its the expected average payoff for infinite paths
\[
\liminf_{T\rightarrow\infty}(T+1)^{-1}\sum_{t=0}^T E[r_i]
\]
where $r_i$ is the immediate reward obtained at step $i$ of the infinite path.\\
\textbf{Total effective payoff:} It is a variant for expected total payoff given by,
\[
\liminf_{T\rightarrow\infty}(T+1)^{-1}\sum_{t=0}^T\sum_{j=0}^t E[r_j]
\]
\\
\textbf{Problem:} Find the maximum possible total effecyive payoff under any strategy\\
It has been shown that memoryless strategy maximizes total effective payoff and this maxima can be found by solving an LP.
\end{enumerate}



\subsection{Stochastic Stability}
\begin{enumerate}
\item \textbf{Title:} On the stability of Stochastic Dynamical Systems (PNAS 1965)\\
\textbf{Author:} Harold J. Kushner\\
\textbf{Summary:}\\
The dynamical model is given by $x_{n+1}=f(x_n,y_n)$ where $y_n$ is a Markov process. Some stability definitions are obtained from here:
\begin{itemize}
\item The origin is stable with probability 1 iff for any $\rho>0$, $\epsilon>0$, there is $\delta(\rho,\epsilon)>0$ 
such that if $\norm{x_0}{}<\delta(\rho,\epsilon)$ then $\prob(\sup_n ||x_n|| \geq\epsilon)\leq\rho$.

\item The origin is asymptotically stable with probability 1 iff it is stable with probability 1 and $x_n$ tends to 0 with probability 1 for all $x_0$ in some neighborhood of the origin.
\end{itemize}

\vspace{10pt}

\item \textbf{Title:} Stability analysis for stochastic hybrid systems: A survey (Automatica 2014)\\
\textbf{Author:} A.R. Teel et. al.\\
\textbf{Summary:}\\
Various SHS have been considered such as Markov jump systems, Switching diffusion system, impulsive system driven by renewal process or Levy diffusion, Stochastic switched and impulsive system etc. 
We get following notions of stochastic stability for these systems:
\begin{itemize}
\item \textbf{Exponential stability:} For a system with solution set $s$, the closed set $A\subset \real^n$ is globally exponentially stable in the $p^{th}$ mean if there exists $k>0$, $\gamma>0$ such that
\[
E[|x(t)|^p_A]\leq k |\xi|^p_A \exp(-\gamma t)
\]
for all $\xi\in\real^n$, $x\in s(\xi)$ and $t\geq 0$.

\item \textbf{Lyapunov stability:} For a system with solution set $s$, the closed set $A \subset \real^n$ is said to be Lyapunov stable in the $p^{th}$ mean ($p>0$) if 
\[
\lim_{i\rightarrow\infty} \sup_{t\geq0} E[|x_i(t)|^p_A] = 0
\]
for each sequence $x_i \in s(\xi_i)$ and each bounded sequence $\xi_i$ satisfying $\lim_{i\rightarrow\infty} |\xi_i|_A = 0$.

\item \textbf{Lagrange stability:} For a system with solution set $s$, the closed set $A \subset \real^n$ is said to be Lagrange stable in the $p^{th}$ mean ($p > 0$), if 
\[
\sup_{t\geq 0} E[|x(t)|^p_A] < \infty \text{ for each }x \in s.
\]

\item \textbf{Asymptotic Stability:} For a system with solution set $s$, the closed set $A \subset \real^n$ is said to be globally attractive in the $p^{th}$ mean if $$\lim_{t \rightarrow\infty} E [|x(t)|^p_A] = 0$$
for each $x \in s$. It is globally asymptotically stable in the $p^{th}$ mean if it is Lyapunov stable in the $p^{th}$ mean, Lagrange stable in the $p^{th}$ mean, and globally attractive in the $p^{th}$ mean.
\end{itemize}
Here the notation $|x|^p_A$ implies $\inf_{y\in A}|x-y|^p$, where $|\cdot|^p$ is the $p^{th}$ mean. Actually it implies the distance of $x$ from the set $A$.
\end{enumerate}

==> dtmc.tex <==
\section{Almost Sure Convergence of WDTMC}\label{sec:dtmc}

Let $(\Mw,\policy)$ be a $\rdtmc$, where $\Mw$ is the $\rmdp$ and $\policy$ is the associated memoryless policy. 
We say a $\rdtmc$ $(\Mw,\policy)$ is almost surely convergent if almost surely all infinite paths have negative mean payoff.
We will first derive a necessary and sufficient condition for almost sure convergence of irreducible $\rdtmc$s, where every state is reachable from every other state. 
We will show that for an irreducible $\rdtmc$, there exists a constant $w$ known as the effective weight of the $\rdtmc$ such that, mean payoff of an infinite path of the $\rdtmc$ is almost surely $w$. 
This constant depends on the stationary distribution of the $\rdtmc$, which is a probability distribution $d^*$ on the set of states $\states$ such that, for all $s\in\states$, 
\[\sum_{(s',\policy(s'),s)\in\edgeset}d^*(s')\trans(s|s',\policy(s'))=d^*(s).\]


%\begin{comment}
We begin by defining a set of random variables $\{X^e_j\mid e\in\edgeset;j\in\nat\}$ on the set of infinite paths of $\Mw$, that captures the information of whether an edge $e\in\edgeset$ appears on the $j^{\textit{th}}$ step of an infinite path $\Path$. More precisely,
\begin{equation*}
	X^e_j(\Path) = 
	\begin{cases}
		W(e) \text{ if }\Path[j:j+1]=e\\
		0 \text{ otherwise}.
	\end{cases}
\end{equation*}
Next, we define partial average weight upto $n$ for an infinite path $\Path$ as
\begin{equation*}
	\frac{\pwavg{n}(\Path)}{n} := \frac{\sum_{i=1}^{n}\weight(\Path[i:i+1])}{n},
\end{equation*}
and note that~\cite{das2022stability},
\begin{equation*}
	\frac{\pwavg{n}(\Path)}{n}=\frac{\sum_{e\in\edgeset}\sum_{j=1}^n X^e_j(\Path)}{n}.
\end{equation*}
Hence, $\{(\pwavg{n}/n)\mid n\in\nat\}$ is a set of random variables on $\ipath{\Mw}$. Note that, for all $\Path\in\ipath{\Mw}$, $\meanpay(\Path)=\limsup_{n\rightarrow\infty}(\pwavg{n}(\Path)/n)$, which is also a random variable on $\ipath{\Mw}$ since it maps $\ipath{\Mw}$ to $\real$.
We now state the following theorem where we show that, an infinite path of an irreducible $\rdtmc$ has a constant mean payoff with probability $1$.
%\end{comment}
\begin{lemma}\label{thm:expct-bdd}
If a $\rdtmc$ $(\Mw,\policy)$ is irreducible, then mean payoff of an infinite path is
\[
w = \sum_{(s,\policy(s),s')\in \edgeset}
d^*(s)\trans(s'|s,\policy(s))\weight_\policy(s,\policy(s),s') \text{ almost surely},
\]
where $d^*$ is the stationary distribution of the $\rdtmc$.
\end{lemma}

\begin{proof}
Note that, since $\rdtmc$ $(\Mw,\policy)$ is irreducible, it has a stationary distribution~\cite{ROSS2010191}. Now suppose, the $\rdtmc$ is periodic (see definition in~\cite{ROSS2010191}) with period $m$. Then, for an edge $e\in \edgeset$ and an infinite path $\Path$,
\begin{align*}
    \frac{\sum_{j=1}^n X^e_j(\Path)}{n}&\leq \frac{\sum_{j=1}^{km} X^e_j(\Path)}{km} + \frac{\sum_{j=km+1}^{km+r}X^e_j(\Path)}{km}\\
    &\ \ \ \ \ \ \ \ 
    [\text{where }r=n\Mod{m}\text{ and }k=(n-r)/m]\\
    &\leq \frac{\sum_{j=1}^{km} X^e_j(\Path)}{km} + \frac{\max_{e\in \edgeset}\weight_\policy(e)}{km}
\end{align*}
since $X^e_j\neq 0$ for at most one $j\in\{km+1,\dots,km+r\}$ as period is $m$. 
Similarly, we can show that,
\[
\frac{\sum_{j=1}^n X^e_j(\Path)}{n}\geq \frac{\sum_{j=1}^{(k+1)m} X^e_j(\Path)}{(k+1)m} - \frac{\max_{e\in \edgeset}\weight_\policy(e)}{(k+1)m}.
\]
Thus,
\begin{align*}
&\lim_{k\rightarrow\infty}\frac{\sum_{j=1}^{(k+1)m} X^e_j(\Path)}{(k+1)m} - \lim_{k\rightarrow\infty}\frac{\max_{e\in \edgeset}\weight_\policy(e)}{(k+1)m}\\
&\leq \limsup_{n\rightarrow\infty}\frac{\sum_{j=1}^n X^e_j(\Path)}{n}\\
&\leq \lim_{k\rightarrow\infty}\frac{\sum_{j=1}^{km} X^e_j(\Path)}{km} + \lim_{k\rightarrow\infty}\frac{\max_{e\in \edgeset}\weight_\policy(e)}{km},\\
& \text{i.e.}, \limsup_{n\rightarrow\infty}\frac{\sum_{j=1}^n X^e_j(\Path)}{n}=\lim_{k\rightarrow\infty}\frac{\sum_{j=1}^{km} X^e_j(\Path)}{km}.
\end{align*}
Since for any edge $e=(s,\policy(s),s')$ of $\edgeset$, 
\begin{align*}
&\lim_{k\rightarrow\infty}\frac{\sum_{j=1}^{km}X^e_j}{km}=d^*(s)\trans(s'|s,\policy(s))\weight_\policy(s,\policy(s),s')\quad\text{almost surely~\cite{das2022stability,ROSS2010191}},\\
\Rightarrow&\limsup_{n\rightarrow\infty}\frac{\sum_{j=1}^n X^e_j}{n} = 
d^*(s)\trans(s'|s,\policy(s))\weight_\policy(s,\policy(s),s')\text{ almost surely}.
\end{align*}
Thus, mean payoff for an infinite path of the $\rdtmc$ is almost surely,
\begin{align*}
&w=\limsup_{n\rightarrow\infty}\frac{\pwavg{n}}{n} = \limsup_{n\rightarrow\infty}\frac{\sum_{e\in \edgeset}\sum_{j=1}^n X^e_j}{n}\\
&=\sum_{e\in \edgeset}\left(\limsup_{n\rightarrow\infty}\frac{\sum_{j=1}^n X^e_j}{n}\right)\\
&= \sum_{(s,s')\in \edgeset}d^*(s)\trans(s'|s,\policy(s))\weight_\policy(s,\policy(s),s').
\end{align*}\qed
\end{proof}


For a state $s$ and a set of states $\B$, we say $\B$ is reachable from $s$ if there exists $s'\in\B$ such that $s'$ is reachable from $s$. 
An infinite path $\Path$ is said to end up in a set of states $\B$, if $\exists n\in\nat$ such that all states in $\Path[n:\infty]$ belongs to $\B$.
For a general $\rdtmc$, an infinite path almost surely ends up  in one of the bottom strongly connected components ($\bscc$s) reachable from $\initst$~\cite{Baier2008}. Note that, a $\bscc$ is a set of states such that, for any state in the set, only states within that set are reachable. 
Let us now show that for any $\bscc$ reachable from $\initst$, there is a non-zero probability that an infinite path ends up in that $\bscc$.

\begin{lemma}\label{lem:end-bscc}
Let $\B$ be a $\bscc$ of a general $\rdtmc$ $(\Mw,\policy)$ such that, $\B$ is reachable from the initialization point $\initst$. Then there is a non-zero probability that an infinite path ends up in $\B$.
\end{lemma}

\begin{proof}
Since $\B$ is reachable from $\initst$, there is a finite path $\pi$ such that $\pi_0=\initst$ and $\pathend{\pi}\in\B$. 
Now, all infinite paths with prefix $\pi$ must end up in $\B$ as it is not possible to leave $\B$ after entering. 
The set of all infinite paths with prefix $\pi$ has probability $\trans_\policy(\pi)>0$~\cite{gimbert2007pure}. 
Thus, an infinite path ends up in $\B$ with probability at least $\trans_\policy(\pi)$, which proves our claim.\qed
\end{proof}

Based on these observations, we can now derive a necessary and sufficient condition for almost sure convergence of a general $\rdtmc$. 
Basically, we can say a $\rdtmc$ is almost surely convergent iff, effective weight of every $\rdtmc$ induced by a $\bscc$ is negative.

\begin{theorem}[Almost Sure Convergence of $\rdtmc$]\label{thm:as-conv-dtmc}
A $\rdtmc$ is almost surely convergent iff effective weight of every $\rdtmc$ induced by a $\bscc$ (reachable from $\initst$) is negative.
\end{theorem}

\begin{proof}
($\Rightarrow$) Suppose a $\rdtmc$ is almost surely convergent.
Then almost surely all infinite paths have negative mean payoff. 
Now, let $\B$ be an arbitrary $\bscc$ reachable from $\initst$. 
Since probability of the set of infinite paths having negative mean payoff is $1$, probability of the set of infinite paths with negative mean payoff given all states are taken from $\B$ is also $1$.
Now the $\rdtmc$ induced by $\B$ is irreducible since $\B$ is a $\bscc$. 
Thus, it has an effective weight (by lemma~\ref{thm:expct-bdd}) and almost surely all infinite paths of it has mean payoff equal to that effective weight. 
This implies, the effective weight of the $\rdtmc$ induced by $\B$ is negative.

($\Leftarrow$) Conversely, let us assume for contradiction that a $\bscc$ reachable from $\initst$ induces a $\rdtmc$ with non-negative effective weight. 
By lemma~\ref{lem:end-bscc}, there is a set of infinite paths of the original $\rdtmc$ that ends up in this $\bscc$ and, probability of this set is greater than $0$. 
Now, almost surely all paths of this set has mean payoff equal to the effective weight of the induced $\rdtmc$.
This is because, almost surely all infinite paths of the induced $\rdtmc$ have mean payoff equal to its effective weight and, the mean payoff of an infinite path does not depend on any of its finite prefix. 
Thus, with non-zero probability, there is a set of infinite paths of the original $\rdtmc$ having non-negative mean payoff, i.e., the original $\rdtmc$ is not almost surely convergent.\qed
\end{proof}

==> lp.tex <==
\section{Finding maximum expected average payoff by LP}

The expected average payoff is given by:
\[
\meanpay(\Path) = \avg\left[\liminf_{n\rightarrow\infty}\frac{\sum_{i=1}^n r_i}{n}\right]
\]
Note that, for a communicating MDP, that is, for any two states $s,s'$, there is a strategy such that $s\reach s'$, the maximum expected average payoff is constant no matter the initialization point. We have the following LP from Puterman1994 that characterizes this value:

\begin{align*}
&\max \sum_{s\in\states}\sum_{a\in\acts}r(s,a)x(s,a)\\
\text{subject to, }&\\
&\sum_{a\in\acts}x(j,a) - \sum_{s\in\states}\sum_{a\in\acts}p(j|s,a)x(s,a) = 0, \quad\forall j\in\states,\\
&\sum_{a\in\acts}x(j,a)+\sum_{a\in\acts}y(j,a)-\sum_{s\in\states}\sum_{a\in\acts}p(j|s,a)y(s,a) = |\states|^{-1}\quad\forall j\in\states\\
& x(s,a)\geq 0\quad\forall s\in\states,\forall a\in\acts\\
& y(s,a)\geq 0\quad\forall s\in\states,\forall a\in\acts.
\end{align*}

Now in general, an MDP may not be communicating. However, we can decompose an MDP into communicating sub MDPs by MEC decomposition (see Krishnendu2011). This is exactly like SCC decomposition for a directed graph. We give the algorithm for MEC decomposition here.

\begin{algorithm}[ht]
\begin{algorithmic}[1]
    \renewcommand{\algorithmicrequire}{\textbf{Input:}}
    \renewcommand{\algorithmicensure}{\textbf{Output:}}
	\Require{A graph $G$ constructed from MDP}
	\Ensure{All MECs of the MDP}
	
	\State $G':= G$
    \State $SCC := ComputeSCCs(G')$
    \While{$\exists$ vertex $(s,a)$ and edge $((s,a),s')$ such that $SCC(a)\neq SCC(s')$}
    \State Remove $(s,a)$ from $G'$
    \State $SCC := ComputeSCCs(G')$
    \EndWhile
\end{algorithmic}
\caption{Algorithm for MEC Decomposition}\label{algo:mec}
\end{algorithm}

Now for each MEC of the MDP we can apply above LP to find the optimal gain. Now for an MEC $M_i$ let,
\begin{align*}
&\submax{r} = \max_{s\in\states,a\in\acts} r(s,a)\text{ and,}\\
&f(M_i) = g^*(M_i)/\submax{r}
\end{align*}
where $g^*(M_i)$ is the optimal gain for the MEC. We construct a new graph from the original MDP where each MEC is a single vertex and from each MEC $M_i$ a new action leads to two new states $s^+$ and $s^-$ with probabilities $f(M_i)$ and $1-f(M_i)$ respectively. This construction is called the MEC quotient of the MDP (see Jan2017). 
On the MEC quotient we have to find the maximum probability of reaching $s^+$, which can be solved by another LP:
\begin{align*}
&\max x(\initst)\\
\text{subject to, }&\\
& x(s) = \sum_{a\in\acts}y(s,a),\quad\forall s\in\states,\\
& x(s,a) = \sum_{s'\in\edgeset(s,a)}y(s,a,s'),\quad\forall (s,a)\in\states\times\acts,\\
& y(s,a,s') = x(s')p(s'|s,a),\quad\forall (s,a,s')\in\edgeset,\\
& x(s^+) = 1,\\
& x(s^-) = 0,\\
& 0\leq x(s)\leq 1,\quad\forall s\in\states,\\
& 0\leq x(s,a)\leq 1,\quad\forall (s,a)\in\states\times\acts,\\
& 0\leq y(s,a)\leq 1,\quad\forall (s,a)\in\states\times\acts,\\
& 0\leq y(s,a,s')\leq 1,\quad\forall (s,a,s')\in\edgeset.
\end{align*}
Here $\edgeset(s,a)$ denotes the set $\{s'\mid p(s'|s,a)>0\}$.

Now let $\submax{p}$ denote the answer to the above LP. Then our required solution is $\submax{p}\cdot\submax{r}$.

==> mdp.tex <==
\section{Almost Sure Convergence of WMDP}\label{sec:mdp}

Now, we will show that it is enough to consider memoryless policies only to decide almost sure convergence of a $\rmdp$. 
Let $\Mw$ be a $\rmdp$. We define random variables $\{X^e_j\mid e\in\edgeset;j\in\nat\}$, $\pwavg{n}/n$ and $\meanpay$ from $\ipath{\Mw}$ to $\real$ as in section~\ref{sec:dtmc}.
We now have the following lemma which states that, the probability of the mean payoff being non-negative is maximized by a memoryless policy.

\begin{lemma}\label{lem:max-prob-mem}
Given a $\rmdp$ $\Mw$, there is a memoryless policy $\optpol$ such that,
\begin{equation*}
\max_{\policy\in\polset}\left[\prob_\policy\left(\limsup_{n\rightarrow\infty}\frac{\pwavg{n}}{n}\geq 0\right)\right]
    =\prob_{\optpol}\left(\limsup_{n\rightarrow\infty}\frac{\pwavg{n}}{n}\geq 0\right).
\end{equation*}
\end{lemma}

\begin{proof}
Let $\dist{\acts}$ denote the set of all distributions on the set of actions of $\Mw$. Suppose, policies are defined as functions from $\fpath{\Mw}$ to $\dist{\acts}$. Note that, for any function $\policy:\fpath{\Mw}\rightarrow\acts$, we can define an equivalent function $\eq{\policy}:\fpath{\Mw}\rightarrow\dist{\acts}$ as,
\[
\eq{\policy}(\Path)(a) = 
\begin{cases}
1 \text{ if }\policy(\Path)=a\\
0 \text{ otherwise.}
\end{cases}
\]
Thus, the above definition encapsulates Definition~\ref{def:policy}. This means, it is sufficient to prove the lemma for policies defined as above.
A policy (defined as above) is positional if it is a memoryless indicator function, i.e., the next distribution of actions is determined based on the current state only and, for each state only one action is chosen with probability $1$. 
A payoff function $\phi$ is prefix-independent if for any $u\in\fpath{\Mw}$ and any $v\in\ipath{\Mw}$, $\phi(uv) = \phi(v)$, and, 
it is submixing if for any infinite sequence of finite paths $u_0,v_0,u_1,v_1,\dots$, $\phi(u_0v_0u_1v_1\dots)\leq\max\{\phi(u_0u_1\dots),\phi(v_0v_1\dots)\}$.
We now state the following theorem from~\cite{gimbert2007pure},
\begin{theorem}\label{thm:pure-stn-opt}
For any prefix-independent and submixing payoff function, there is a positional policy that maximizes the expectation of the payoff function.
\end{theorem}
Let us define a payoff function $\phi:\ipath{\Mw}\rightarrow\{0,1\}$ as,
\[
\phi(\Path) = 
\begin{cases}
1 \text{ if }\meanpay(\Path)\geq 0\\
0 \text{ otherwise.}
\end{cases}
\]
Note that, for any $u\in\fpath{\Mw}$ and $v\in\ipath{\Mw}$,
$\phi(uv) = 1$ iff 
$\meanpay(uv)\geq 0$ iff 
$\meanpay(v)\geq 0$ iff 
$\phi(v)=1$, since mean payoff $\meanpay$ is prefix-independent. 
Hence, $\phi$ is prefix-independent. 
Similarly, for any infinite sequence of finite paths $u_0,v_0,u_1,v_1,\dots$,
\begin{align*}
&\phi(u_0v_0u_1v_1\dots) = 1\\
\Rightarrow & \meanpay(u_0v_0u_1v_1\dots)\geq 0\\
\Rightarrow & \meanpay(u_0u_1\dots)\geq 0 \text{ or }\meanpay(v_0v_1\dots)\geq 0\quad
\text{(since }\meanpay\text{ is submixing)}\\
\Rightarrow & \phi(u_0u_1\dots)=1 \text{ or } \phi(v_0v_1\dots)=1.
\end{align*}
Hence, $\phi(u_0v_0u_1v_1\dots)\leq\max\{\phi(u_0u_1\dots),\phi(v_0v_1\dots)\}$, i.e., $\phi$ is submixing. This implies, by Theorem~\ref{thm:pure-stn-opt}, the existence of a positional policy $\optpol$ that maximizes the expectation of $\phi$, that is,
\[
\max_{\policy\in\polset}\avg^\policy[\phi]=\avg^{\optpol}[\phi].
\]
Now since $\phi$ is a Bernoulli random variable on the set of infinite paths $\ipath{\Mw}$, $\avg^\policy[\phi]=\prob_\policy(\phi=1)$ for all $\policy\in\polset$. Thus,
\begin{align*}
&\max_{\policy\in\polset}\avg^\policy[\phi] = \max_{\policy\in\polset}\prob_\policy(\phi=1)
=\max_{\policy\in\polset}\prob_\policy(\meanpay\geq 0)\\
&= \max_{\policy\in\polset}\left[\prob_\policy\left(\limsup_{n\rightarrow\infty}\frac{\pwavg{n}}{n}\geq 0\right)\right]\\
&= \avg^{\optpol}[\phi]=\prob_{\optpol}(\phi=1)
=\prob_{\optpol}(\meanpay\geq 0)\\
&= \prob_{\optpol}\left(\limsup_{n\rightarrow\infty}\frac{\pwavg{n}}{n}\geq 0\right).
\end{align*}
Since $\optpol$ is positional, it has an equivalent deterministic representation (as in Definition~\ref{def:policy}). Thus, there exists a memoryless policy (as in Definition~\ref{def:policy}) which maximizes the probability of $\{\Path\in\ipath{\Mw}\mid\pwavg{n}(\Path)/n\geq 0\}$.\qed
\end{proof}


We can now provide a necessary and sufficient condition for almost sure convergence of $\rmdp$ based on Lemma~\ref{lem:max-prob-mem}. Basically, we can say a $\rmdp$ is almost surely convergent if and only if for any memoryless policy, probability of $\{\Path\in\ipath{\Mw}\mid\pwavg{n}(\Path)/n\geq 0\}$ is less or equal to zero.
\begin{theorem}\label{thm:suff-conv}
A $\rmdp$ $\Mw$ is almost surely convergent if and only if for any memoryless policy $\memless{\policy}$, 
\[
\prob_{\memless{\policy}}\left(\limsup_{n\rightarrow\infty}\frac{\pwavg{n}}{n}\geq 0\right)\leq 0
\]
\end{theorem}
\begin{proof}
We know from Lemma~\ref{lem:max-prob-mem} that, probability of $\{\Path\in\ipath{\Mw}\mid\pwavg{n}(\Path)/n\geq 0\}$ is maximized by a memoryless policy. Let $\memless{\polset}$ be the set of all memoryless policies. Then there exists $\optpol\in\memless{\polset}$ such that,
\[
\max_{\policy\in\polset}\left[\prob_\policy\left(\limsup_{n\rightarrow\infty}\frac{\pwavg{n}}{n}\geq 0\right)\right]
    =\prob_{\optpol}\left(\limsup_{n\rightarrow\infty}\frac{\pwavg{n}}{n}\geq 0\right).
\]
Thus, by definition of almost sure convergence, $\Mw$ is almost surely convergent if and only if,
\begin{align*}
&\prob_{\policy}\{\Path\in\ipath{\Mw}\mid\meanpay(\Path)<0\}=1\quad\forall\policy\in\polset\\
\text{iff, }&\prob_\policy\{\Path\in\ipath{\Mw}\mid\pwavg{n}(\Path)/n\geq 0\}\leq 0 \quad\forall\policy\in\polset\\
\text{iff, }&\max_{\policy\in\polset}\left[\prob_\policy\left(\limsup_{n\rightarrow\infty}\frac{\pwavg{n}}{n}\geq 0\right)\right]\leq 0\\
\text{iff, }&\max_{\policy\in\memless{\polset}}\left[\prob_\policy\left(\limsup_{n\rightarrow\infty}\frac{\pwavg{n}}{n}\geq 0\right)\right]\leq 0\\
\text{iff, }&\prob_\policy\{\Path\in\ipath{\Mw}\mid\pwavg{n}(\Path)/n\geq 0\}\leq 0 \quad\forall\policy\in\memless{\polset}.
\end{align*}\qed
\end{proof}
